Simpson's Paradox in Recommender Fairness: Reconciling differences between per-user and aggregated evaluations

There has been a flurry of research in recent years on notions of fairness in ranking and recommender systems, particularly on how to evaluate if a recommender allocates exposure equally across groups of relevant items (also known as provider fairness). While this research has laid an important foundation, it gave rise to different approaches depending on whether relevant items are compared per-user/per-query or aggregated across users. Despite both being established and intuitive, we discover that these two notions can lead to opposite conclusions, a form of Simpson's Paradox. We reconcile these notions and show that the tension is due to differences in distributions of users where items are relevant, and break down the important factors of the user's recommendations. Based on this new understanding, practitioners might be interested in either notions, but might face challenges with the per-user metric due to partial observability of the relevance and user satisfaction, typical in real-world recommenders. We describe a technique based on distribution matching to estimate it in such a scenario. We demonstrate on simulated and real-world recommender data the effectiveness and usefulness of such an approach.

==> Fairness metrics in Recs (e2e, confound) (4)/proof.tex <==
\textbf{Step 1: Exposure of relevant (vs irrelevant) items on a given user.} 

The performance controls how the total exposure available (noted as ExposureAvailable) is allocated to relevant/irrelevant items, as we see in the following equations (using the definition of Performance).

For a given user $u$,
\begin{align*}
\begin{split}
ExposureAvailable =& \ (Comp_0(u) + Comp_1(u)) * \mathop{{}\mathbb{E}}_i [Exposure(i, u) | Rel(i,u) = 1] \\
&+ (|I| - Comp_0(u) - Comp_1(u)) *
\mathop{{}\mathbb{E}}_i [Exposure(i, u) | Rel(i,u) = 0] \\
%\end{split}
%\end{align*}
%\begin{align*}
%\begin{split}
ExposureAvailable =& \ |I| * \mathop{{}\mathbb{E}}_i [Exposure(i, u) | Rel(i,u) = 1] \\
&- (|I| - Comp_0(u) - Comp_1(u)) * Performance(u)
\end{split}
\end{align*}

Finally, we have:
\begin{align*}
\begin{split}
\mathop{{}\mathbb{E}}_i [Exposure(i, u) | Rel(i,u) = 1] =& \ \frac{ExposureAvailable}{|I|} \\
&+ (1 - \frac{Comp_0(u) + Comp_1(u))}{|I|}) * Performance(u)) 
\end{split}
\end{align*}

\vspace{5mm}
\textbf{Step 2: Exposure of relevant items from a given group on a given user.}

The expected exposure of relevant content is a weighted sum over the exposure of the two groups. The following equations follow (using the definition of Per-user Gap).

For a given user $u$,
\begin{align*}
%\begin{equation}
\begin{split}
\mathop{{}\mathbb{E}}_i [Exposure(i, u) | Rel(i,u) = 1] =& \
  \frac{Comp_1(u)}{Comp_1(u) + Comp_0(u)} * \mathop{{}\mathbb{E}}_i [Exp(i,u) | Rel(i,u) = 1, S = 1] \\
& + \frac{Comp_0(u)}{Comp_1(u) + Comp_0(u)} * \mathop{{}\mathbb{E}}_i [Exp(i,u) | Rel(i,u) = 1, S = 0] \\ 
% New line below
 \mathop{{}\mathbb{E}}_i [Exposure(i, u) | Rel(i,u) = 1] =& \ \mathop{{}\mathbb{E}}_i [Exp(i,u) | Rel(i,u) = 1, S = 1]  - \frac{Comp_0(u)}{Comp_1(u) + Comp_0(u)} * PerUserGap(u)
\end{split}
%\end{equation}
\end{align*}

\vspace{5mm}
Finally we have:

\begin{align*}
\begin{split}
\mathop{{}\mathbb{E}}_i [Exposure(i, u) | Rel(i,u) = 1, S = 1] = & \ [Exposure(i, u) | Rel(i,u) = 1] + \frac{Comp_0(u)}{Comp_1(u) + Comp_0(u)} * PerUserGap(u)
\end{split}
\end{align*}


This equation is relatively intuitive. If there is no per-context bias, the relevant content from the sensitive group will get the same exposure. Otherwise, the exposure might be higher or lower depending on the bias.

%\vspace{5mm}
We can then write the exposure of a given group as a function of the per-user bias, the performance and the competition.

\begin{align*}
\begin{split}
\mathop{{}\mathbb{E}}_i [Exposure(i, u) | Rel(i,u) = 1, S = 1]
= & \ \frac{ExposureAvailable}{|I|} \\
&+ (1 - \frac{Comp_0(u) + Comp_1(u)}{|I|}) * Performance(u)\\
&+ \frac{Comp_0(u)}{Comp_1(u) + Comp_0(u)} * PerUserGap(u)
\end{split}
\end{align*}


\vspace{50mm}
\textbf{Step 3: Gap aggregated across users.}

\begin{align*}
\begin{split}
AggregateGap =&  \ \frac{1}{\sum_{u} Comp_1(u)} \sum_{u} Comp_1(u) * \mathop{{}\mathbb{E}}_i [Exposure(i, u) | Rel(i,u) = 1, S = 1] \\
&- \frac{1}{\sum_{u} Comp_0(u)} \sum_{u} Comp_0(u) * \mathop{{}\mathbb{E}}_i [Exposure(i, u) | Rel(i,u) = 1, S = 0] \\
%\end{split}
%\end{align*}
%
%\begin{align*}
%\begin{split}
AggregateGap =& \ \sum_{u} \Biggl(\\
\frac{Comp_1(u)}{\sum_{u} Comp_1(u)} * \biggl(
&\frac{ExposureAvailable}{|I|}
+ (1 - \frac{Comp_0(u) + Comp_1(u)}{|I|}) * Performance(u)
+ \frac{Comp_0(u)}{Comp_1(u) + Comp_0(u)} * PerUserGap(u)\biggr) \\
- \frac{Comp_0(u)}{\sum_{u} Comp_0(u)} * \biggl(
&\frac{ExposureAvailable}{|I|}
+ (1 - \frac{Comp_0(u) + Comp_1(u)}{|I|}) * Performance(u)
- \frac{Comp_1(u)}{Comp_1(u) + Comp_0(u)} * PerUserGap(u)\biggr) \Biggr) \\
%\end{split}
%\end{align*}
%\begin{align*}
%\begin{split}
AggregateGap =& \ \sum_{u} \Biggl(\\
&\frac{ExposureAvailable}{|I|} * \biggl(\frac{Comp_1(u)}{\sum_{u} Comp_1(u)} - \frac{Comp_0(u)}{\sum_{u} Comp_0(u)}  \biggr) \\
& + Performance(u) * \biggl(\frac{Comp_1(u)}{\sum_{u} Comp_1(u)} - \frac{Comp_0(u)}{\sum_{u} Comp_0(u)} \biggr) * \biggl(1 - \frac{Comp_0 (u) + Comp_1 (u)}{|I|} \biggr) \\
& + PerUserGap(u) * \biggl(\frac{Comp_1(u)}{\sum_{u} Comp_1(u)}  * \frac{Comp_0(u)}{Comp_1(u) + Comp_0(u)} + \frac{Comp_0(u)}{\sum_{u} Comp_0(u)} * \frac{Comp_1(u)}{Comp_1(u) + Comp_0(u)} \biggr) \Biggr) \\
%\end{split}
%\end{align*}
%\begin{align*}
%\begin{split}
AggregateGap =& \ \sum_{u} \Biggl(\\
& + Performance(u) * \biggl(\frac{ Comp_1(u)}{\sum_{u} Comp_1(u)} - \frac{Comp_0(u)}{\sum_{u} Comp_0(u)}\biggr) * \biggl(1 - \frac{Comp_0 (u) + Comp_1 (u)}{|I|} \biggr) \\
& + PerUserGap(u) * \biggl(\frac{1}{\sum_{u} Comp_1(u)} + \frac{1}{\sum_{u} Comp_0(u)} \biggr) * \frac{Comp_0(u) * Comp_1(u)}{Comp_1(u) + Comp_0(u)} \Biggr) \\
\end{split}
\end{align*}



% Option 1:
% \begin{align*}
% \begin{split}
% AggregateGap =& \ \sum_{u} \Biggl(\\
% &\frac{Comp_1(u)}{\sum_{u} Comp_1(u)} * \biggl( \\
% &\frac{ExposureAvailable}{|I|}
% + (1 - \frac{Comp_0(u) + Comp_1(u)}{|I|}) * Performance(u)
% + \frac{Comp_0(u)}{Comp_1(u) + Comp_0(u)} * PerUserGap(u)\biggr) \\
% & - \frac{Comp_0(u)}{\sum_{u} Comp_0(u)} * \biggl( \\
% &\frac{ExposureAvailable}{|I|}
% + (1 - \frac{Comp_0(u) + Comp_1(u)}{|I|}) * Performance(u)
% - \frac{Comp_1(u)}{Comp_1(u) + Comp_0(u)} * PerUserGap(u)\biggr) \Biggr) \\
% \end{split}
% \end{align*}

% Option 2:
% \begin{align*}
% \begin{split}
% AggregateGap =& \ \sum_{u} \Biggl(\\
% \frac{Comp_1(u)}{\sum_{u} Comp_1(u)} * \biggl(
% &\frac{ExposureAvailable}{|I|}
% + (1 - \frac{Comp_0(u) + Comp_1(u)}{|I|}) * Performance(u)
% + \frac{Comp_0(u)}{Comp_1(u) + Comp_0(u)} * PerUserGap(u)\biggr) \\
% - \frac{Comp_0(u)}{\sum_{u} Comp_0(u)} * \biggl(
% &\frac{ExposureAvailable}{|I|}
% + (1 - \frac{Comp_0(u) + Comp_1(u)}{|I|}) * Performance(u)
% - \frac{Comp_1(u)}{Comp_1(u) + Comp_0(u)} * PerUserGap(u)\biggr) \Biggr) \\
% \end{split}
% \end{align*}



% \clearpage
% \newpage
% \newpage
% \newpage
% Interpretation:

% Let the relative relevance ($RR_i(u)$) of a given user $u$ be the number of relevant items for group $i$ for $u$ divided by the total number of relevant items for group $i$ across all users:
% \begin{align*}
% \begin{split}
% RR_i(u) &= \frac{ Comp_i(u)}{\sum_{u} Comp_i(u)}
% \end{split}
% \end{align*}

% Let the relative relevance difference ($RRD(u)$) of a given user $u$ be the difference in relative relevances between the two groups:
% \begin{align*}
% \begin{split}
% RRD(u) &= RR_1(u) - RR_0(u)
% &= \frac{ Comp_1(u)}{\sum_{u} Comp_1(u)} - \frac{ Comp_0(u)}{\sum_{u} Comp_0(u)}
% \end{split}
% \end{align*}

% Let $NR(u)$ be the fraction of non-relevant items for user $u$:
% \begin{align*}
% \begin{split}
% NR(u) &= 1 - \frac{Comp_0 (u) + Comp_1 (u)}{|I|}
% \end{split}
% \end{align*}

% Furthermore, let $Z$ be the following constant:
% \begin{align*}
% \begin{split}
% Z &= \frac{1}{\sum_{u} Comp_1(u)} - \frac{1}{\sum_{u} Comp_0(u)}
% \end{split}
% \end{align*}

% Then the Aggregate Gap is:
% \begin{align*}
% \begin{split}
% AggregateGap &= \sum_{u} \Biggl(\\
% &\frac{ExposureAvailable}{|I|} * RRD(u) \\
% & + Performance(u) * RRD(u) * NR(u) \\
% & + PerUserGap(u) * Z * \frac{Comp_0(u) * Comp_1(u)}{Comp_1(u) + Comp_0(u)} \Biggr) \\
% \end{split}
% \end{align*}

% Thus, each user's contribution to the Aggregate Gap is composed of three factors:
% \begin{itemize}
%     \item The available exposure for that user times its relative relevance difference
%     \item The performance for that user times its relative relevance difference
%     \item The bias for that user times a constant times a factor that depends on the number of relevant items from each group (and is largest when the groups are balanced)
% \end{itemize}

% Some observations:
% \begin{itemize}
%     \item When Performance and Bias are 0, there can still be an aggregate gap
% \end{itemize}
